Segment Any Class (SAC): Multi-Class Few-Shot Semantic Segmentation via Class Region Proposals

The Segment-Anything Model (SAM) is a vision foundation model for segmentation with a prompt-driven framework. SAM generates class-agnostic masks based on user-specified instance-referring prompts. However, adapting SAM for automated segmentation -- where manual input is absent -- of specific object classes often requires additional model training. We present Segment Any Class (SAC), a novel, training-free approach that task-adapts SAM for Multi-class segmentation. SAC generates Class-Region Proposals (CRP) on query images which allows us to automatically generate class-aware prompts on probable locations of class instances. CRPs are derived from elementary intra-class and inter-class feature distinctions without any additional training. Our method is versatile, accommodating any N-way K-shot configurations for the multi-class few-shot semantic segmentation (FSS) task. Unlike gradient-learning adaptation of generalist models which risk the loss of generalization and potentially suffer from catastrophic forgetting, SAC solely utilizes automated prompting and achieves superior results over state-of-the-art methods on the COCO-20i benchmark, particularly excelling in high N-way class scenarios. SAC is an interesting demonstration of a prompt-only approach to adapting foundation models for novel tasks with small, limited datasets without any modifications to the foundation model itself. This method offers interesting benefits such as intrinsic immunity to concept or feature loss and rapid, online task adaptation of foundation models.

==> figures/cluster_num.tex <==
\begin{figure}[H]
  \centering
   \includegraphics[width=0.95\linewidth]{figures/cluster_num.png}
   \caption{Cluster number, increasing cluster number up to a point saturates mIoU}
   \label{fig:cluster_num}
\end{figure}

==> figures/mask_filter.tex <==
\begin{figure}[H]
  \centering
   \includegraphics[width=0.95\linewidth]{figures/mask_filter.png}
   \caption{Mask Filtering. Class region overlap is calculated for each mask and if it scores below threshold, the mask is filtered out}
   \label{fig:mask_filter}
\end{figure}

==> figures/mccsam.tex <==
\begin{figure*}
  \centering
   \includegraphics[width=0.9\linewidth]{figures/mccsam.png}
   \caption{An overview of MCC-SAM}
   \label{fig:mccsam}
\end{figure*}

==> figures/qualitative_domain.tex <==
\begin{figure*}
  \centering
   \includegraphics[width=0.75\linewidth]{figures/qualitative_domain.png}
   \caption{Qualitative results of 6-way and 7-way 1-shot segmentation on LoveDA and SUIM dataset respectively. Displayed from left to right are the following: Ground Truth, SAC prediction, and Class Region Proposal.}
   \label{fig:qualitative_domain}
\end{figure*}

==> tables/datasets.tex <==
\begin{table}[!ht]
    \centering
    \caption{Datasets used for evaluation}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccccccc}
    \hline
        \textbf{\#} & \textbf{Dataset} & \textbf{Domain} & \textbf{Support Pool \#} \\ \hline
        1 & LoveDA\cite{Wang2021LoveDA:Segmentation} & Remote Sensing & 1366(rural) \\ 
         ~ & ~ & ~ & 1156(urban) \\ 
        2 & BUSI\cite{Al-Dhabyani2020DatasetImages} & Medical & 323 \\ 
        3 & SUIM\cite{Islam2020SemanticBenchmark} & Underwater & 762 \\ 
        4 & PCB\_det\cite{PCB_Component_Detection} & Industrial & 1099 \\ \hline
    \end{tabular}
    }
    \label{tab:datasets}
\end{table}

==> tables/diff_class.tex <==
\begin{table}[!ht]
\centering
\caption{Class-pairing evaluation of mccsam}
\begin{tabular}{c|c}
Support Class & Fish mIoU \\ \hline
No support    & 0.371     \\
Plants        & 0.415     \\
Ruins         & 0.391     \\
Robots        & 0.402     \\
Reefs         & 0.428     \\
Diver         & 0.402     \\
Rocks         & 0.384    
\end{tabular}

\label{tab:diff_class}
\end{table}

==> tables/domain.tex <==
\begin{table}[H]
\centering
\caption{SAC N-way 1-shot on selected datasets}
\scalebox{1.3}{
\begin{tabular}{c|c|l}
Dataset        & N-way & mIoU \\ \hline
LoveDA (rural) & 6     & 22.81    \\
LoveDA (urban) & 6     & 30.91     \\
SUIM           & 7     & 39.57   
\end{tabular}
}
\label{tab:domain}
\end{table}

==> tables/extractor.tex <==
\begin{table}[H]
\centering
\scalebox{1.4}{
\begin{tabular}{c|c}
network   &      \\ \hline
SAM    & 26.6 \\
DINOv2 & 45.5
\end{tabular}
}
\caption{Network used to extract support features to produce CRFAs}
\label{tab:extractor}
\end{table}

==> tables/kway.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{test}
\scalebox{1.4}{
\begin{tabular}{cccccc|ccccc}
\hline
\multirow{2}{*}{Method} & \multicolumn{5}{c|}{2-way 1-shot} & \multicolumn{5}{c}{5-way 1-shot} \\ \cline{2-11} 
 &
  \multicolumn{1}{c|}{fold-0} &
  \multicolumn{1}{c|}{fold-1} &
  \multicolumn{1}{c|}{fold-2} &
  \multicolumn{1}{c|}{fold-3} &
  mean &
  \multicolumn{1}{c|}{fold-0} &
  \multicolumn{1}{c|}{fold-1} &
  \multicolumn{1}{c|}{fold-2} &
  \multicolumn{1}{c|}{fold-3} &
  mean \\ \hline
\multicolumn{1}{c|}{LA} &
  \multicolumn{1}{c|}{31.0} &
  \multicolumn{1}{c|}{38.2} &
  \multicolumn{1}{c|}{34.7} &
  \multicolumn{1}{c|}{34.5} &
  34.6 &
  \multicolumn{1}{c|}{24.2} &
  \multicolumn{1}{c|}{27.5} &
  \multicolumn{1}{c|}{29.6} &
  \multicolumn{1}{c|}{29.7} &
  27.7 \\
\multicolumn{1}{c|}{SAC} &
  \multicolumn{1}{c|}{39.8} &
  \multicolumn{1}{c|}{49.6} &
  \multicolumn{1}{c|}{49.2} &
  \multicolumn{1}{c|}{48.0} &
  46.6 &
  \multicolumn{1}{c|}{39.3} &
  \multicolumn{1}{c|}{47.3} &
  \multicolumn{1}{c|}{48.1} &
  \multicolumn{1}{c|}{41.5} &
  44.0
\end{tabular}
}

\label{tab:kway}
\end{table*}

==> tables/multi_class.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table}[!ht]
% \centering
% \caption{}
% \begin{tabular}{c|c|ccc}
% Dataset &          & \textbf{}                         & \textbf{} & \textbf{} \\ \hline
%         & Building & 0.295                             & 0.318     & 0.357     \\
%         & Road     & \cellcolor[HTML]{656565}\textbf{} & 0.343     & 0.376     \\
% \multirow{-3}{*}{LoveDA (Urban)} & Water  & \cellcolor[HTML]{656565}\textbf{} & \cellcolor[HTML]{656565}\textbf{} & 0.394 \\
%         & Fish     & 0.371                             & 0.384     & 0.42      \\
%         & Rocks    & \cellcolor[HTML]{656565}\textbf{} & 0.301     & 0.297     \\
% \multirow{-3}{*}{SUIM}           & Plants & \cellcolor[HTML]{656565}\textbf{} & \cellcolor[HTML]{656565}\textbf{} & 0.082
% \end{tabular}
% \label{tab:multi_class}
% \end{table}


\begin{table}[!ht]
\centering
\caption{Multiclass evaluation of mccsam}
\label{tab:multi_class}
\begin{tabular}{c|c|ccc}
Dataset &          & \textbf{1-class}                         & \textbf{2-class} & \textbf{3-class} \\ \hline
        & Building & 0.295                             & 0.318     & 0.357     \\
        & Road     & \cellcolor[HTML]{B7B7B7}\textbf{} & 0.343     & 0.376     \\
\multirow{-3}{*}{LoveDA (Urban)} & Water  & \cellcolor[HTML]{B7B7B7}\textbf{} & \cellcolor[HTML]{B7B7B7}\textbf{} & 0.394 \\ \hline
        & Fish     & 0.371                             & 0.384     & 0.42      \\
        & Rocks    & \cellcolor[HTML]{B7B7B7}\textbf{} & 0.297     & 0.301     \\
\multirow{-3}{*}{SUIM}           & Plants & \cellcolor[HTML]{B7B7B7}\textbf{} & \cellcolor[HTML]{B7B7B7}\textbf{} & 0.082
\end{tabular}%

\end{table}


==> tables/prompting.tex <==
\begin{table}[!ht]
\centering
\caption{mIoU results of prompting methods}
\label{tab:prompting}
\scalebox{1.2}{
\begin{tabular}{l|ll}
               & \multicolumn{1}{l|}{Naive} & Guided \\ \hline
LoveDA (rural) & 0.530                      & 0.609  \\
LoveDA (urban) & 0.636                      & 0.674  \\
BUSI           & 0.190                      & 0.518  \\
SUIM           & 0.732                      & 0.786  \\
PCB\_det       & 0.858                      & 0.894 
\end{tabular}
}
\end{table}

==> tables/quantitative.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\caption{quantitative evaluation of mccsam on semantic segmentation}
\label{tab:quantitative}
\begin{tabular}{c|c|ccc|c|cccc}
Dataset &
  classes &
  \begin{tabular}[c]{@{}c@{}}MCC-SAM\\ (upper limit)\end{tabular} &
  MCC-SAM &
  Segformer-B5 &
  Dataset &
  \multicolumn{1}{c|}{classes} &
  \begin{tabular}[c]{@{}c@{}}MCC-SAM\\ (upper limit)\end{tabular} &
  MCC-SAM &
  Segformer-B5 \\ \hline
\multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}LoveDA \\ (Rural)\end{tabular}} &
  Building &
  0.550 &
  0.408 &
  0.204 &
  \multirow{7}{*}{\begin{tabular}[c]{@{}c@{}}LoveDA \\ (Urban)\end{tabular}} &
  \multicolumn{1}{c|}{Building} &
  0.610 &
  0.408 &
  0.298 \\
 &
  Road &
  0.551 &
  0.345 &
  0.052 &
   &
  \multicolumn{1}{c|}{Road} &
  0.561 &
  0.395 &
  0.375 \\
 &
  Water &
  0.810 &
  0.259 &
  0.334 &
   &
  \multicolumn{1}{c|}{Water} &
  0.833 &
  0.504 &
  0.534 \\
 &
  Barren &
  0.567 &
  0.040 &
  0.057 &
   &
  \multicolumn{1}{c|}{Barren} &
  0.701 &
  0.079 &
  0.105 \\
 &
  Forest &
  0.378 &
  0.059 &
  0.045 &
   &
  \multicolumn{1}{c|}{Forest} &
  0.614 &
  0.279 &
  0.325 \\
 &
  Agriculture &
  0.799 &
  0.441 &
  0.399 &
   &
  \multicolumn{1}{c|}{Agriculture} &
  0.727 &
  0.143 &
  0.244 \\ \cline{2-5} \cline{7-10} 
 &
  \textbf{Mean} &
  \textbf{0.609} &
  \textbf{0.259} &
  \textbf{0.182} &
   &
  \multicolumn{1}{c|}{\textbf{Mean}} &
  \textbf{0.674} &
  \textbf{0.301} &
  \textbf{0.313} \\ \hline
\multirow{9}{*}{PCB\_det} &
  Cap1 &
  0.950 &
  0.807 &
  0.924 &
  \multirow{9}{*}{SUIM} &
  \multicolumn{1}{c|}{Diver} &
  0.789 &
  0.563 &
  0.786 \\
 &
  Cap2 &
  0.894 &
  0.866 &
  0.902 &
   &
  \multicolumn{1}{c|}{Plants} &
  0.652 &
  0.058 &
  0.186 \\
 &
  Cap3 &
  0.950 &
  0.622 &
  0.944 &
   &
  \multicolumn{1}{c|}{Ruins} &
  0.817 &
  0.261 &
  0.782 \\
 &
  Cap4 &
  0.930 &
  0.495 &
  0.909 &
   &
  \multicolumn{1}{c|}{Robots} &
  0.814 &
  0.609 &
  0.684 \\
 &
  MOSFET &
  0.942 &
  0.767 &
  0.920 &
   &
  \multicolumn{1}{c|}{Reefs} &
  0.824 &
  0.410 &
  0.752 \\
 &
  Mov &
  0.807 &
  0.562 &
  0.942 &
   &
  \multicolumn{1}{c|}{Fish} &
  0.818 &
  0.518 &
  0.747 \\
 &
  Resistor &
  0.907 &
  0.552 &
  0.747 &
   &
  \multicolumn{1}{c|}{Rocks} &
  0.789 &
  0.267 &
  0.542 \\
 &
  Transformer &
  0.770 &
  0.699 &
  0.861 &
   &
  \multicolumn{1}{c|}{\textbf{}} &
  \textbf{} &
  \textbf{} &
  \textbf{} \\ \cline{2-5} \cline{7-10} 
 &
  \textbf{Mean} &
  \textbf{0.894} &
  \textbf{0.684} &
  \textbf{0.893} &
   &
  \multicolumn{1}{c|}{\textbf{Mean}} &
  \textbf{0.786} &
  \textbf{0.384} &
  \textbf{0.640} \\ \hline
BUSI &
  Cancer &
  \textbf{0.518} &
  \textbf{0.412} &
  \textbf{0.733} &
   &
   &
   &
   &
  
\end{tabular}
\end{table*}
